Should one compute the Temporal Difference fix point or minimize the Bellman Residual? The unified oblique projection view

We investigate projection methods, for evaluating a linear approximation of the value function of a policy in a Markov Decision Process context. We consider two popular approaches, the one-step Temporal Difference fix-point computation (TD(0)) and the Bellman Residual (BR) minimization. We describe examples, where each method outperforms the other. We highlight a simple relation between the objective function they minimize, and show that while BR enjoys a performance guarantee, TD(0) does not in general. We then propose a unified view in terms of oblique projections of the Bellman equation, which substantially simplifies and extends the characterization of (schoknecht,2002) and the recent analysis of (Yu & Bertsekas, 2008). Eventually, we describe some simulations that suggest that if the TD(0) solution is usually slightly better than the BR solution, its inherent numerical instability makes it very bad in some cases, and thus worse on average.

==> rbf_200ech_br_vk_g0.95.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(6480.00,4032.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(1210,440){\makebox(0,0)[r]{\strut{} 0}}%
      \put(1210,1106){\makebox(0,0)[r]{\strut{} 0.2}}%
      \put(1210,1771){\makebox(0,0)[r]{\strut{} 0.4}}%
      \put(1210,2437){\makebox(0,0)[r]{\strut{} 0.6}}%
      \put(1210,3102){\makebox(0,0)[r]{\strut{} 0.8}}%
      \put(1210,3768){\makebox(0,0)[r]{\strut{} 1}}%
      \put(1342,220){\makebox(0,0){\strut{} 0}}%
      \put(1943,220){\makebox(0,0){\strut{} 20}}%
      \put(2544,220){\makebox(0,0){\strut{} 40}}%
      \put(3145,220){\makebox(0,0){\strut{} 60}}%
      \put(3745,220){\makebox(0,0){\strut{} 80}}%
      \put(4346,220){\makebox(0,0){\strut{} 100}}%
      \put(4947,220){\makebox(0,0){\strut{} 120}}%
      \put(5548,220){\makebox(0,0){\strut{} 140}}%
      \put(6149,220){\makebox(0,0){\strut{} 160}}%
      \put(440,2104){\rotatebox{90}{\makebox(0,0){\strut{}Distance à l'optimal}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(5162,3595){\makebox(0,0)[r]{\strut{}0.0}}%
      \csname LTb\endcsname%
      \put(5162,3375){\makebox(0,0)[r]{\strut{}0.1}}%
      \csname LTb\endcsname%
      \put(5162,3155){\makebox(0,0)[r]{\strut{}0.3}}%
      \csname LTb\endcsname%
      \put(5162,2935){\makebox(0,0)[r]{\strut{}0.5}}%
      \csname LTb\endcsname%
      \put(5162,2715){\makebox(0,0)[r]{\strut{}0.7}}%
      \csname LTb\endcsname%
      \put(5162,2495){\makebox(0,0)[r]{\strut{}0.8}}%
      \csname LTb\endcsname%
      \put(5162,2275){\makebox(0,0)[r]{\strut{}0.9}}%
      \csname LTb\endcsname%
      \put(5162,2055){\makebox(0,0)[r]{\strut{}0.95}}%
      \csname LTb\endcsname%
      \put(5162,1835){\makebox(0,0)[r]{\strut{}1.0}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{rbf_200ech_br_vk_g0.95.eps}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> rbf_200ech_fp_vk_g0.95.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(6480.00,4032.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(1210,440){\makebox(0,0)[r]{\strut{} 0}}%
      \put(1210,1106){\makebox(0,0)[r]{\strut{} 0.2}}%
      \put(1210,1771){\makebox(0,0)[r]{\strut{} 0.4}}%
      \put(1210,2437){\makebox(0,0)[r]{\strut{} 0.6}}%
      \put(1210,3102){\makebox(0,0)[r]{\strut{} 0.8}}%
      \put(1210,3768){\makebox(0,0)[r]{\strut{} 1}}%
      \put(1342,220){\makebox(0,0){\strut{} 0}}%
      \put(1943,220){\makebox(0,0){\strut{} 20}}%
      \put(2544,220){\makebox(0,0){\strut{} 40}}%
      \put(3145,220){\makebox(0,0){\strut{} 60}}%
      \put(3745,220){\makebox(0,0){\strut{} 80}}%
      \put(4346,220){\makebox(0,0){\strut{} 100}}%
      \put(4947,220){\makebox(0,0){\strut{} 120}}%
      \put(5548,220){\makebox(0,0){\strut{} 140}}%
      \put(6149,220){\makebox(0,0){\strut{} 160}}%
      \put(440,2104){\rotatebox{90}{\makebox(0,0){\strut{}Distance à l'optimal}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(5162,3595){\makebox(0,0)[r]{\strut{}0.0}}%
      \csname LTb\endcsname%
      \put(5162,3375){\makebox(0,0)[r]{\strut{}0.1}}%
      \csname LTb\endcsname%
      \put(5162,3155){\makebox(0,0)[r]{\strut{}0.3}}%
      \csname LTb\endcsname%
      \put(5162,2935){\makebox(0,0)[r]{\strut{}0.5}}%
      \csname LTb\endcsname%
      \put(5162,2715){\makebox(0,0)[r]{\strut{}0.7}}%
      \csname LTb\endcsname%
      \put(5162,2495){\makebox(0,0)[r]{\strut{}0.8}}%
      \csname LTb\endcsname%
      \put(5162,2275){\makebox(0,0)[r]{\strut{}0.9}}%
      \csname LTb\endcsname%
      \put(5162,2055){\makebox(0,0)[r]{\strut{}0.95}}%
      \csname LTb\endcsname%
      \put(5162,1835){\makebox(0,0)[r]{\strut{}1.0}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{rbf_200ech_fp_vk_g0.95.eps}}%
    \gplfronttext
  \end{picture}%
\endgroup

